J-PLUS DR3: Galaxy-Star-Quasar classification

The Javalambre Photometric Local Universe Survey (J-PLUS) is a 12-band photometric survey using the 83-cm JAST telescope. Data Release 3 includes 47.4 million sources. J-PLUS DR3 only provides star-galaxy classification so that quasars are not identified from the other sources. Given the size of the dataset, machine learning methods could provide a valid alternative classification and a solution to the classification of quasars. Our objective is to classify J-PLUS DR3 sources into galaxies, stars and quasars, outperforming the available classifiers in each class. We use an automated machine learning tool called TPOT to find an optimized pipeline to perform the classification. The supervised machine learning algorithms are trained on the crossmatch with SDSS DR18, LAMOST DR8 and Gaia. We checked that the training set of about 660 thousand galaxies, 1.2 million stars and 270 thousand quasars is both representative and contain a minimal presence of contaminants (less than 1%). We considered 37 features: the twelve photometric bands with respective errors, six colors, four morphological parameters, galactic extinction with its error and the PSF relative to the corresponding pointing. With TPOT genetic algorithm, we found that XGBoost provides the best performance: the AUC for galaxies, stars and quasars is above 0.99 and the average precision is above 0.99 for galaxies and stars and 0.96 for quasars. XGBoost outperforms the classifiers already provided in J-PLUS DR3 and also classifies quasars.

==> authorlist.tex <==
\author{
R.~von~Marttens\inst{\ref{instRvM1},\ref{instRvM2},\ref{instRvM3}}
\and
V.~Marra\inst{\ref{instVM1},\ref{instVM2},\ref{instVM3}}\thanks{E-mail address: valerio.marra@inaf.it}
\and
M.~Quartin\inst{\ref{instMQ1},\ref{instMQ2},\ref{instMQ3}}
\and
L.~Casarini\inst{\ref{instLC}}
\and
P.~O.~Baqui\inst{\ref{instPB}}
\and
A. Alvarez-Candal\inst{\ref{inst1},\ref{inst2},\ref{instRvM2}}
\and
F. J. Galindo-Guil\inst{\ref{inst3}}
\and
J.A. Fernández-Ontiveros\inst{\ref{inst3}}
\and
Andrés del Pino\inst{\ref{inst3}}
\and
L.A. D\'iaz-Garc\'ia\inst{\ref{inst5}}
\and
C. L\'opez-Sanjuan\inst{\ref{inst4}}
\and
J.~Alcaniz\inst{\ref{instRvM2}}
\and
R.~Angulo\inst{\ref{inst11},\ref{inst12}}
\and
A.~J.~Cenarro\inst{\ref{inst4}}
\and
D.~Cristóbal-Hornillos\inst{\ref{inst3}}
\and
R.~Dupke\inst{\ref{instRvM2}, \ref{inst8}, \ref{inst9}}
\and
A.~Ederoclite\inst{\ref{inst10}}
\and
C.~Hernández-Monteagudo\inst{\ref{inst4}, \ref{inst6}, \ref{inst7}}
\and
A.~Marín-Franch\inst{\ref{inst4}}
\and
M.~Moles\inst{\ref{inst3}}
\and
L.~Sodré\inst{\ref{inst10}}
\and
J.~Varela\inst{\ref{inst4}}
\and
H.~Vázquez Ramió\inst{\ref{inst4}}
}

\institute{\small
Instituto de Física, Universidade Federal da Bahia, 40210-340, Salvador-BA, Brasil \label{instRvM1}
\and
PPGCosmo, Universidade Federal do Espírito Santo, 29075-910, Vitória, ES, Brazil \label{instRvM2}
\and
Observat\'orio Nacional, Rua General Jos\'e Cristino 77, Rio de Janeiro, RJ, 20921-400, Brazil \label{instRvM3}
\and
Departamento de Física, Universidade Federal do Espírito Santo, 29075-910, Vitória, ES, Brazil \label{instVM1}
\and
INAF -- Osservatorio Astronomico di Trieste, via Tiepolo 11, 34131 Trieste, Italy \label{instVM2}
\and
IFPU -- Institute for Fundamental Physics of the Universe, via Beirut 2, 34151, Trieste, Italy \label{instVM3}
\and
Instituto de Física, Universidade Federal do Rio de Janeiro, 21941-972, Rio de Janeiro, RJ, Brazil \label{instMQ1}
\and
Observatório do Valongo, Universidade Federal do Rio de Janeiro, 20080-090, Rio de Janeiro, RJ, Brazil \label{instMQ2}
\and
Institute of Theoretical Physics, Heidelberg University, Philosophenweg 16, 69120 Heidelberg, Germany \label{instMQ3}
\and
Departamento de Física, Universidade Federal de Sergipe, 49100-000, Aracaju, SE, Brazil \label{instLC}
\and
Núcleo Cosmo-ufes, Universidade Federal do Espírito Santo, 29075-910, Vitória, ES, Brazil \label{instPB}
\and
Instituto de Astrof\'isica de Andaluc\'ia, CSIC, Apt 3004, E18080 Granada, Spain \label{inst1}
\and
Instituto de F\'isica Aplicada a las Ciencias y las Tecnolog\'ias, Universidad de Alicante, San Vicent del Raspeig, E03080, Alicante, Spain \label{inst2}
\and
Centro de Estudios de F\'isica del Cosmos de Arag\'on (CEFCA), Plaza San Juan 1, 44001 Teruel, Spain \label{inst3}
\and
Instituto de Astrof\'isica de Andaluc\'ia (IAA-CSIC), P.O.~Box 3004, 18080 Granada, Spain \label{inst5}
\and
Centro de Estudios de F\'isica del Cosmos de Arag\'on (CEFCA), Unidad Asociada al CSIC, Plaza San Juan 1, 44001 Teruel, Spain \label{inst4}
\and
Donostia International Physics Center (DIPC),  Manuel Lardizabal Ibilbidea, 4, San Sebasti\'an, Spain \label{inst11}
\and
Ikerbasque, Basque Foundation for Science, E-48013 Bilbao \label{inst12}
\and
Department of Astronomy, University of Michigan, 311West Hall, 1085 South University Ave., Ann Arbor, USA \label{inst8}
\and
Department of Physics and Astronomy, University of Alabama, Box 870324, Tuscaloosa, AL, USA \label{inst9}
\and
Departamento de Astronomia, Instituto de Astronomia, Geofísica e Ciências Atmosféricas, Universidade de São Paulo, 05508-090, São Paulo, SP, Brazil \label{inst10}
\and
Instituto de Astrof\'isica de Canarias, C/ V\'ia L\'actea, s/n, E-38205, La Laguna, Tenerife, Spain \label{inst6}
\and
Departamento de Astrof\'isica, Universidad de La Laguna, E-38206, La Laguna, Tenerife, Spain \label{inst7}
}






















